Automatic Recall Machines: Internal Replay, Continual Learning and the Brain

Replay in neural networks involves training on sequential data with memorized samples, which counteracts forgetting of previous behavior caused by non-stationarity. We present a method where these auxiliary samples are generated on the fly, given only the model that is being trained for the assessed objective, without extraneous buffers or generator networks. Instead the implicit memory of learned samples within the assessed model itself is exploited. Furthermore, whereas existing work focuses on reinforcing the full seen data distribution, we show that optimizing for not forgetting calls for the generation of samples that are specialized to each real training batch, which is more efficient and scalable. We consider high-level parallels with the brain, notably the use of a single model for inference and recall, the dependency of recalled samples on the current environment batch, top-down modulation of activations and learning, abstract recall, and the dependency between the degree to which a task is learned and the degree to which it is recalled. These characteristics emerge naturally from the method without being controlled for.

==> figs/densities_combined.tex <==
\begin{figure}[b]
     %\hspace*{-0.8em}%
     \setlength{\belowcaptionskip}{-0.3em}
     \includegraphics[width=0.3125\textwidth]{imgs/recall_density_cifar10_Blues_r_3703.png}%
     \includegraphics[width=0.3125\textwidth]{imgs/recall_density_cifar10_Blues_r_3707.png}%
     \includegraphics[width=0.375\textwidth]{imgs/recall_density_cifar10_Blues_r_3719.png}
%\setlength{\belowcaptionskip}{-1.5em}
\caption{
History of recalled classes throughout training for different diversity weights $\lambda_3$. 
Vertical slices denote $\frac{1}{M} \sum_{\hat{x} \in \mathcal{\hat{B}}_X} f_{\theta}(\hat{x})$ per training timestep.
Current training classes (diagonal) are not recalled due to non-locality~(\cref{e:kp_orig}).
Unseen tasks (lower triangle) are naturally avoided.
}
\label{f:densities_combined}
\end{figure}

\begin{comment}
\begin{figure}[b]
     \hspace*{-0.8em}%
     \setlength{\belowcaptionskip}{-0.3em}
     \subfloat[][CIFAR10]{
     \includegraphics[width=0.23\textwidth]{imgs/recall_density_cifar10_Blues_r_3703.png}
     \includegraphics[width=0.23\textwidth]{imgs/recall_density_cifar10_Blues_r_3707.png}
     \includegraphics[width=0.276\textwidth]{imgs/recall_density_cifar10_Blues_r_3719.png}
     \label{f:densities1}
     }\hspace*{-0.8em}%
     \setlength{\belowcaptionskip}{-0.3em}
     \subfloat[][MiniImageNet]{
     \includegraphics[width=0.255\textwidth]{imgs/recall_density_miniimagenet_Blues_r_4825.png}
     \label{f:densities2}
     }
\end{figure}
\end{comment}

==> figs/fig_accuracy_recall_corr.tex <==
\begin{figure}
\centering
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/accuracy_recall_corr_mnist.png}
  \caption{MNIST}
  %\label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/accuracy_recall_corr_cifar10.png}
  \caption{CIFAR10}
  %\label{fig:sub2}
\end{subfigure}%
\begin{subfigure}{.32\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/accuracy_recall_corr_miniimagenet.png}
  \caption{MiniImageNet}
  \label{f:}
\end{subfigure}
\caption{
Recall and training accuracy after training on a task are positively correlated across datasets, heavily supported by the first task which is strongly recalled and performed in all cases (top right corner).
Dashed line denotes best linear fit with least squares.
}
\label{f:accuracy_recall_corr}
\end{figure}



==> figs/fig_accuracy_with_divs.tex <==
\begin{figure}
\centering
\includegraphics[width=0.35\linewidth]{imgs/accuracy_with_divs.png}
\caption{
Relative accuracy of \methodnameshort with different values of diversity weight $\lambda_3$.
The optimal value of $\lambda_3$ is negatively correlated with the number of classes in a dataset.
}
\label{f:accuracy_with_divs}
\end{figure}

==> figs/fig_new_splash.tex <==
\begin{figure}
\centering
%\includegraphics[width=0.99\linewidth]{imgs/new_splash_wide}
\includegraphics[width=0.8\linewidth]{imgs/new_splash.png}
%\setlength{\belowcaptionskip}{-1em}
\caption{\methodname. The model trains on real $\mathcal{B}$ while generating and reinforcing maximally interfered $\mathcal{\hat{B}}$ from its implicit memory.
%the model trains on real $\mathcal{B}$ while generating and reinforcing maximally interfered $\mathcal{\hat{B}}$ from its implicit memory.
%At $t=0$, randomly initialized $f_{\theta'} = f_{\theta}$.
In each stage, the model or recalled samples (green) are optimized for objective (blue) and updated (red).
The change in predictions
%on inputs $\mathcal{\hat{B}}_X$
between old $f_{\theta}$ and new $f_{\theta'}$ is maximised by $\operatorname{recall}$~(\cref{e:recall}).
Reinforcing the resulting maximally interfered
%non-local 
$\mathcal{\hat{B}}_X$ with old outputs from $f_{\theta}$ optimally minimizes forgetting of $f_{\theta'}$,
%latter, 
because in theory if the maximal divergence between old and new non-local behavior is 0, then all such divergences are 0. 
Thus training on $\mathcal{B}$ updates local behavior while training on $\mathcal{\hat{B}}$ protects behavior in the rest of input space.
}
\label{f:splash}
\end{figure}

==> figs/fig_recall_density_cifar10.tex <==
\begin{figure}
\centering
\includegraphics[width=\linewidth]{imgs/recall_density_cifar10_Blues_r_three.png}
\caption{\methodnameshort on CIFAR10: history of recalled classes throughout training for different diversity weight $\lambda_3$; $\lambda_3=16$ yields best performance.
5 tasks are formed from adjacent pairs of classes.
Color denotes $\frac{1}{M} \sum_{\hat{x} \in \mathcal{\hat{B}}} f_{\theta}(\hat{x})$ for a given class at a given training timestep.
Recall begins from end of 1st task~\citep{aljundi2019online}.
The classes for the task currently being trained are not recalled (diagonal) due to non-locality of recall~(\cref{e:recall}).
Unseen tasks (lower triangle) are naturally avoided~(\cref{s:avoid_unseen}).
}
\label{f:recall_prog_cifar10}
\end{figure}

==> figs/fig_recall_density_miniimagenet.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\linewidth]{imgs/recall_density_miniimagenet_Blues_r_4825.png}
\caption{\methodnameshort on MiniImageNet: history of recalled classes for best value of $\lambda_3=1$.
20 tasks are formed from 5 adjacent classes each.
Format is same as~\cref{f:recall_prog_cifar10}.
}
\label{f:recall_prog_miniimagenet}
\end{figure}
